HERMES: Scalable, Secure, and Privacy-Enhancing Vehicle Access System

We propose HERMES, a scalable, secure, and privacy-enhancing system for users to share and access vehicles. HERMES securely outsources operations of vehicle access token generation to a set of untrusted servers. It builds on an earlier proposal, namely SePCAR [1], and extends the system design for improved efficiency and scalability. To cater to system and user needs for secure and private computations, HERMES utilizes and combines several cryptographic primitives with secure multiparty computation efficiently. It conceals secret keys of vehicles and transaction details from the servers, including vehicle booking details, access token information, and user and vehicle identities. It also provides user accountability in case of disputes. Besides, we provide semantic security analysis and prove that HERMES meets its security and privacy requirements. Last but not least, we demonstrate that HERMES is efficient and, in contrast to SePCAR, scales to a large number of users and vehicles, making it practical for real-world deployments. We build our evaluations with two different multiparty computation protocols: HtMAC-MiMC and CBC-MAC-AES. Our results demonstrate that HERMES with HtMAC-MiMC requires only approx 1,83 ms for generating an access token for a single-vehicle owner and approx 11,9 ms for a large branch of rental companies with over a thousand vehicles. It handles 546 and 84 access token generations per second, respectively. This results in HERMES being 696 (with HtMAC-MiMC) and 42 (with CBC-MAC-AES) times faster compared to in SePCAR for a single-vehicle owner access token generation. Furthermore, we show that HERMES is practical on the vehicle side, too, as access token operations performed on a prototype vehicle on-board unit take only approx 62,087 ms.

==> Security_Proofs_highlevel.tex <==
\section{Security and Privacy Analysis}\label{sec:analysis}
We prove that \system\ satisfies the security and privacy requirements of Sect.~\ref{sec:system_model}, provided that its underlying cryptographic primitives are sufficiently secure. The theorem statement and the proof given below are informal, in a similar sense by~\cite{DBLP:conf/esorics/SymeonidisAMMDP17}. A complete formal description of the semantic security models and the stand-alone proofs are given in the online version of the system~\cite{HERMES_full}.

\begin{theorem}
Assume that communication takes place over private channels. If:
\begin{itemize}
\item the \gls{MPC} is statistically secure~\cite{rotaru2017modes},
\item the signature scheme $\mathsf{sign}$ is multi-key existentially unforgeable~\cite{DBLP:journals/siamcomp/GoldwasserMR88},
\item the key derivation function $\mathsf{kdf}$ is multi-key secure~\cite{DBLP:journals/jacm/GoldreichGM86},
\item the public-key encryption scheme $\mathsf{enc}$ is multi-key semantically secure~\cite{DBLP:conf/eurocrypt/BellareBM00},
\item the symmetric key encryption scheme $\mathsf{E}$ is multi-key chosen-plaintext secure~\cite{DBLP:conf/focs/BellareDJR97},
% \item \textcolor{red}{Bart: fix this} the authenticated encryption scheme $\mathsf{auth}$ is multi-key secure~\cite{DBLP:journals/joc/BellareN08},
\item the hash function $\mathsf{hash}$ is collision resistant~\cite{DBLP:conf/fse/RogawayS04}, and
\item the \gls{MAC} function $\mathsf{mac}$ is multi-key existentially unforgeable~\cite{DBLP:journals/siamcomp/GoldwasserMR88},
\end{itemize}
then \system\ fulfills the security and privacy requirements of Sect.~\ref{sec:system_model}.
\end{theorem}
Note that, indeed, for each of the keyed cryptographic primitives we require security in the \emph{multi-key} setting, as these are evaluated under different keys. For example, $\mathsf{sign}$ is used by all owners, each with a different key; $\mathsf{enc}$ is used for different keys, each for a different party in the \gls{VSSP}, and $\mathsf{E}$ and $\mathsf{mac}$ are used for independent keys (i.e., session keys) for every fresh evaluation of the protocol. We refer to Bellare et al.~\cite{DBLP:conf/eurocrypt/BellareBM00} for a discussion on generalizing semantic security of public-key encryption to multi-key security; the adaptation straightforwardly generalizes to the other security models. 
\begin{proof}[Proof sketch]
We treat the security and privacy requirements, and discuss how these are achieved from the cryptographic primitives, separately. We recall that the consumer and owner have agreed upon the booking details prior to evaluating \system. Hence they know each other.

\paragraph{SR1 -- Confidentiality of $M^B$} In one evaluation of the protocol, $u_c$, $u_o$, and the shared vehicle learn the booking details by default or design. The \gls{VSSP} servers only learn shares of the booking data, and under the assumption that the \gls{MPC} is statistically secure, nothing about the booking data is revealed during the \gls{MPC}. The outcomes of the \gls{MPC} are $AuthTag^{M_B}$ and $C^{u_c}$ satisfying

\begin{align}
&AuthTag^{M_B} = \mathsf{mac}(K^{u_c}_{tag_{mac}},\mathsf{E}(K^{u_c}_{tag_{enc}},M^{B}))\,,\label{eqn:AuthT}\\
&C^{u_c} = \mathsf{E}(K_{enc}^{u_c},\{\mathsf{E}(K^{veh_{u_o}}_y,\{M^{B},\sigma^{u_o}\}),ID^{veh_{u_o}}\})\,,\label{eqn:Cuc}
\end{align}
both of which reveal nothing about $M^B$ to a malicious outsider due to the assumed security of $\mathsf{mac}$, $\mathsf{E}$, and the independent uniform drawing of the keys $K^{u_c}_{enc}$ and $\vec{K}^{u_c}_{tag}=(K^{u_c}_{tag_{enc}}, K^{u_c}_{tag_{mac}})$. The nested encryption $\mathsf{E}$ does not influence the analysis due to the mutual independence of the keys $K_{enc}^{u_c}$ and $K^{veh_{u_o}}_y$.

\paragraph{SR2 -- Authenticity of $M^B$} An owner who initiates the \gls{AT} generation and distribution, first signs the booking details using its private key before sending those to the \gls{VSSP} in shares. Therefore, once the vehicle receives the token and obtains the booking details, it can verify the owner's signature on the booking details. In other words, the vehicle can verify the source of the booking details, the owner, and their integrity. Suppose, to the contrary, that a malicious consumer can get access to a vehicle of an owner $u_o$. This particularly means that it created a tuple $(M^B,\sigma^{u_o})$ such that $\mathsf{verify}(Pk^{u_o},M^B,\sigma^{u_o})$ holds. If $\sigma^{u_o}$ is new, this means that $u_c$ forges a signature for the secret signing key $\mathit{Sk}^{u_o}$. This is impossible by the assumption that the signature scheme is existentially unforgeable. On the other hand, if $(M^B,\sigma^{u_o})$ is old but the evaluation is fresh, this means a collision $\mathsf{hash}(\mathit{Cert}^{u_c})=\mathsf{hash}(\mathit{Cert}^{u_c\prime})$, which is computationally infeasible as $\mathsf{hash}$ is collision-resistant.

\paragraph{SR3 -- Confidentiality of $AT^{veh_{u_o}}$} The \gls{AT} is generated by the \gls{VSSP} servers obliviously (as the \gls{MPC} is statistically secure), and only revealed to the public in encrypted form, through $C^{u_c}$ of (\ref{eqn:Cuc}). Due to the uniform drawing of the key $K_{enc}^{u_c}$ (and the security of the public-key encryption scheme used to transmit this key), only the legitimate user can decrypt and learn the \gls{AT}. It shares it with the vehicle over a secure and private channel.

\paragraph{SR4 -- Confidentiality of $K^{veh_{u_o}}$} Only the vehicle manufacturer and the vehicle itself hold copies of the vehicle key. Considering the \gls{VM} as a \acrfull{TP}, it holds all the secret keys of vehicles that produce. The \gls{VSSP} servers learn these in shared form, hence learn nothing about it by virtue of the statistical security of the \gls{MPC}. Retrieving a vehicle key from encryptions made under this key constitutes a key recovery attack, which in turn allows breaking the chosen-plaintext security of the symmetric key encryption scheme.

%  By vehicle owners registering their vehicles, the \gls{VSSP} forwards the list of each vehicle key, i.,e $K^{veh_{u_o}}$ to $\mathsf{S}_i$ servers in secret shared form. Thus, no one including the \gls{PD} of the vehicle owner, but \gls{VM} and the vehicle holds the vehicle key.

\paragraph{SR5 -- Backward and forward secrecy of $AT^{veh_{u_o}}$} The \gls{AT} is published on the \acrfull{PL} as $C^{u_c}$ of (\ref{eqn:Cuc}), encrypted under symmetric key $K_{enc}^{u_c}$. Every honest consumer generates a fresh key $K_{enc}^{u_c}$ for every new evaluation. It uses a key derivation function $\mathsf{kdf}$ utilizing a \gls{PRF} for each key generation and every new evaluation of the protocol, and that is secure. This implies that all session keys are drawn independently and uniformly at random. In addition, the symmetric encryption scheme $\mathsf{E}$ is multi-key secure. Concluding, all encryptions $C^{u_c}$ are independent and reveal nothing of each other. Note that nothing can be said about \glspl{AT} for malicious users who may deviate from the protocol and reuse one-time keys.

\paragraph{SR6 -- Non-repudiation of origin of $AT^{veh_{u_o}}$} The vehicle, which is a trusted entity, verifies the origin through verification of the signature, $\mathsf{verify}(Pk^{u_o},M^B,\sigma^{u_o})$. The consumer $u_c$ verifies the origin through the verification of the \gls{MAC} function, i.e., $AuthTag^{M_B} \stackrel{?}{=} \mathsf{mac}(K^{u_c}_{tag_{mac}}, E(K^{u_c}_{tag_{enc}}, M^{B}))$. Note that $u_c$ does not effectively verify $AT^{veh_{u_o}}$, but rather $AuthTag^{M_B}$, which suffices under the assumption that the \gls{MPC} servers evaluate their protocol correctly. In either case, security fails only if the asymmetric signature scheme or the $\mathsf{mac}$ function are forgeable.

\paragraph{SR7 -- Non-repudiation of delivery of $AT^{veh_{u_o}}$} The owner can verify the correct delivery of $AT^{veh_{u_o}}$ with the successful verification and message sent by the vehicle to the owner, $\mathsf{verify}(Pk^{veh_{u_o}},\{M^B,TS^{veh_{u_o}}_{Access}\}, \sigma^{veh_{u_o}}_{Access})$ at the end of the protocol. Security breaks only if the signature scheme is forgeable.

\paragraph{SR8 -- Accountability of users (i.e., owners, and consumers)} In the case of disputes, the information related to a specific transaction (and only this information) may need to be reconstructed. Reconstruction can be done only if the \gls{VSSP} servers collude and reveal their shares. In our setting, these servers have competing interests. Thus they would not collude unless law authorities' request. Due to threshold secret sharing properties, the private inputs can be reconstructed by a majority coalition. This is, if the \gls{VSSP} consists of three parties, it suffices two of party-shares required to reconstruct the secret.

% \paragraph{FR1 -- Accountability of users (i.e., owners, and consumers)}

% % In the case of disputes, the information related to a specific transaction (and only this information) may need to be reconstructed. Reconstruction can be done only if the \gls{VSSP} servers collude and reveal their shares. In our setting, these servers have competing interests. Thus they would not collude unless law authorities' request. Due to threshold secret sharing properties, the private inputs can be reconstructed by a majority coalition. This is, if the \gls{VSSP} consists of three parties, it suffices two of party-shares required to reconstruct the secret.

% In case of incidents and upon requests from authorities, the information related to a specific transaction can be reconstructed; and only that information. Reconstruction can be achieved by the accord of all \gls{VSSP} parties, i.e., $\mathsf{S}_i$, relinquishing their shares to the authority requesting the information validation. In our setting, these servers have competing interests. Thus they would not collude unless law authorities' request. Furthermore, due to threshold secret sharing properties the private inputs can be reconstructed by a majority coalition. Given our three party configuration, it suffices two of such parties inputs, i.e., $\mathsf{S}_i$ to reconstruct the secrets (for the semi-honest and malicious cases). Our system design is agnostic towards the underlying \gls{MPC} building blocks, though. Hence, by replacing~\cite{DBLP:conf/ccs/ArakiFLNO16} and Shamir's sharing mechanism to e.g, SPDZ~\cite{DBLP:conf/esorics/DamgardKLPSS13}, secrets would need the involvement of every \gls{VSSP} server for the reconstruction. %Hence, \system\ satisfies FR1. %\textbf{CHECK: added}

\paragraph{PR1 -- Unlinkability of any two requests of $u_c$ for any $veh_{u_o}$(s)} The only consumer-identifiable data is in the consumer's certificate included in the booking details. Note that these are agreed upon and between the consumer and the owner, so the owner learns the consumer's identity by default. Beyond that, the consumer only communicates with the vehicle, which is supposed to learn the consumer's identity to perform proper access verification. The consumer consults the \gls{PL} over an anonymous communication channel~\cite{torproject}. The booking details are transferred to and from the \gls{VSSP}, but these are encrypted and do not leak by virtue of their confidentiality (security requirement SR1).

\paragraph{PR2 -- Anonymity of $u_c$ and the $veh_{u_o}$} The reasoning is identical to that of PR1.

\paragraph{PR3 -- Indistinguishability of $AT^{veh_{u_o}}$ operations} Access token generation, update, or revocation is performed using the same steps and the same type of messages sent to the \gls{VSSP} and \gls{PL}. Hence, outsiders and system entities cannot distinguish which operation has been requested.
\end{proof}

==> experiments/cbc-vs-htmac.tex <==
\begin{figure}[H]% [h!tb] 
  \centering
  \scalebox{.70}{%
    \begin{tikzpicture}
      %\pgfplotsset{every axis legend/.append style={at={(0.5,1.1)},anchor=south}}
      \begin{axis}[
        tick pos = left,
        %xtick align = outside,
        legend style   = {cells={anchor=west}},
        legend pos = outer north east,
        legend entries = {
          % {$\F_{2^k}$, 1 thread},
          {CBC-MAC-AES},
          {HtMAC MiMC},
        },
        ylabel         = {Communication cost (kB)},
        xlabel         = {Number of vehicles per owner},
        ymode=log,
        xmode=log,
        log basis y={10},
        ]
        \addplot table[x=cars, y=comms] {experiments/cbc-comm};
        \addplot table[x=cars, y=comms] {experiments/htmac-comm};
      \end{axis}
    \end{tikzpicture}
  }
  \caption{Communication cost per server: access token generation cost (i.e., data sent-received) for a number of vehicles per owner.}
  \label{fig:hermes-comm}
\end{figure}

\begin{figure}[H]% [h!tb] 
  \centering
  \scalebox{.70}{%
    \begin{tikzpicture}
      %\pgfplotsset{every axis legend/.append style={at={(0.5,1.1)},anchor=south}}
      \begin{axis}[
        tick pos = left,
        %xtick align = outside,
        legend style   = {cells={anchor=west}},
        legend pos = outer north east,
        legend entries = {
          % {$\F_{2^k}$, 1 thread},
          {CBC-MAC-AES},
          {HtMAC MiMC},
        },
        ylabel         = {Throughput (ops/sec)},
        xlabel         = {Number of vehicles per owner},
        ymode=log,
        xmode=log,
        log basis y={10},
        ]
        \addplot table[x=cars, y=tru] {experiments/cbc-comm};
        \addplot table[x=cars, y=tru] {experiments/htmac-comm};
      \end{axis}
    \end{tikzpicture}
  }
  \caption{Throughput for all servers: access token generation (i.e., ops) per second for a number of vehicles per owner.}
  \label{fig:hermes-tru}
\end{figure}

% \begin{figure*}\label{fig:sims-er}
%     \centering
%   \begin{subfigure}[b]{0.45\textwidth}
%         \begin{tikzpicture}
%       %\pgfplotsset{every axis legend/.append style={at={(0.5,1.1)},anchor=south}}
%       \begin{axis}[
%         tick pos = left,
%         %xtick align = outside,
%         legend style   = {cells={anchor=west}},
%         legend pos = outer north east,
%         legend entries = {
%           % {$\F_{2^k}$, 1 thread},
%           {CBC-MAC-AES},
%           {HtMAC MiMC},
%         },
%         ylabel         = {Total comm (kb)},
%         xlabel         = {Number of vehicles},
%         ymode=log,
%         xmode=log,
%         log basis y={10},
%         ]
%         \addplot table[x=cars, y=comms] {experiments/cbc-comm};
%         \addplot table[x=cars, y=comms] {experiments/htmac-comm};
%       \end{axis}
%     \end{tikzpicture}
%         \caption{Communication sent per party for a query with various Vehicles.}
%         \label{fig:hermes-comm}
%     \end{subfigure}
%     \begin{subfigure}[b]{0.45\textwidth}
%          \begin{tikzpicture}
%       %\pgfplotsset{every axis legend/.append style={at={(0.5,1.1)},anchor=south}}
%       \begin{axis}[
%         tick pos = left,
%         %xtick align = outside,
%         legend style   = {cells={anchor=west}},
%         legend pos = outer north east,
%         legend entries = {
%           % {$\F_{2^k}$, 1 thread},
%           {CBC-MAC-AES},
%           {HtMAC MiMC},
%         },
%         ylabel         = {(ops/s)},
%         xlabel         = {Number of Vehicles},
%         ymode=log,
%         xmode=log,
%         log basis y={10},
%         ]
%         \addplot table[x=cars, y=tru] {experiments/cbc-comm};
%         \addplot table[x=cars, y=tru] {experiments/htmac-comm};
%       \end{axis}
%     \end{tikzpicture}
%         \caption{Degree distribution}
%         \label{fig:hermes-tru}
%     \end{subfigure}
%     \caption{Query throughput with various vehicles.}
% \end{figure*}




==> results.tex <==

% \textcolor{blue}{Summary of efficiency/scalability:
% Application on car-fleet companies / or in general vehicular - overall (user + cars per user) / in comparison SePCAR
% \begin{itemize}
%     \item One table in comparison with SepCAR - 1 Eq. check / avg. on 1000 operations (Step 2) - Can we get SePCAR numbers?
%     \item Communication overhead:
%     \begin{itemize}
%         \item Communication rounds / data / throughput / \textbf{time} 
%         \item Breaking down Step 2: Eq. check \# of ID / Encryptions / EtA
%         \begin{itemize}
%             \item power of 2? 
%         \end{itemize}
%         \item \# of operations - avg. of 1000 evaluations?
%         \item In total / Per server
%     \end{itemize}
%     \item I can work on the plots - needs a .CSV or .Json file
%     \item Are the values on table updated/final?
% \end{itemize}}
%\textcolor{blue}{[IR] latency? (online phase - Step 2)}


%\textcolor{blue}{[MM] Ideally, we need to demonstrate the improvement with regards to SePCAR. I think below we only have the two new implementations of the protocol. Can we have a row for SePCAR too? So, we end up having three protocols for comparison: SePCAR, New protocol (with CBC-MAC-AES) and New Protocol (with HtMAC-MiMC).}

%\textcolor{blue}{[MM] We will have to produce some figures based on the results from the table. Reviewers of IEEE Transactions really like seeing some plots. :)}

%\textcolor{blue}{[MM] maybe we need some numbers in the range between 4 and 256 IDs. Now the switch looks to drastic.}

% \begin{table*}[h!]
% % Centered 'X' column type for tabularx
%   \caption {\system\ performance, i.e., access token generation, per number of vehicles utilizing: CBC-MAC-AES and HtMAC-MiMC. Throughput is evaluated for all servers and communication cost per server.}
%   \label{tab:dabit}
% \newcolumntype{C}{>{\centering\arraybackslash}X}
% \begin{center}
% %   \scalebox{0.9}{
% %   \begin{table}[ht]
%   \begin{tabularx}{\textwidth}{lCCCCC}
% % \begin{tabular}{CCCCCC}
%     \toprule
%   Type of Vehicle Owners & Protocol            & Number of Vehicles per Owner & Communication Rounds & Communication Data (kB) & Throughput (ops/s) \\
% 	\midrule
%      & CBC-MAC-AES & 1   & 568 & 64 & 33 \\ % c =  2, b =  3
%     & HtMAC-MiMC        & 1 & 167 & 108 & 546 \\
% % 	\midrule
%     \cmidrule{2-6}
%     \multirow{3}{*}{Individuals} & CBC-MAC-AES & 2 &  568 & 64 & 32 \\ % c =  2, b =  3
%     & HtMAC-MiMC        & 2  & 167 & 108 & 546 \\
%     \cmidrule{2-6}
% % 	\midrule
%     & CBC-MAC-AES & 4 &  568 &  107.7 & 32 \\ % c =  2, b =  3
%     & HtMAC-MiMC        & 4  & 167 & 117 & 544 \\
%     % \cline{2-6}
% 	\midrule
%     % \cline{2-6}
%      & CBC-MAC-AES & 256 & 568 &  76 & 32 \\ % c =  2, b =  3 
%     & HtMAC-MiMC  & 256  & 167 & 150 & 260 \\
%     %\cline{2-6}
%     \cmidrule{2-6}
%     % \midrule
%     \multirow{3}{*}{Vehicle-rental company branches} & CBC-MAC-AES & 512 & 568 &  88 & 32 \\ % c =  2, b =  3
%     & HtMAC-MiMC  & 512 & 167 & 194 & 151 \\

%     %\midrule
%     \cmidrule{2-6}
%     %\cline{2-6}
%     & CBC-MAC-AES & 1024 & 568 & 112 & 32 \\ % c =  2, b =  3
%     & HtMAC-MiMC  & 1024 & 167 & 280 & 84 \\
 
%     \bottomrule
% %   \end{tabular}
% \end{tabularx}
% %   }
% %   \end{table}
% \end{center}
% \end{table*}

% \input{experiments/cbc-vs-htmac}

% Notes:
% Improved protocol - scalability to multiple cars - evaluations per protocol commence 
% CBC-MAC-AES is now 30 times better than previous evaluation
% With HtMAC, same parameters as previous evaluation we get 500x improvement in throughput
% We also scale to 1024 cars and prove that the scalability of the MPC protocol
% HtMAC is always better than CBC-MAC using the new comparison protocol (see Escudero et al).

%\begin{table*}[htb]
%% Centered 'X' column type for tabularx
%\newcolumntype{C}{>{\centering\arraybackslash}X}
%\begin{center}
%  \scalebox{0.9}{
%  \begin{tabularx}{\textwidth}{CCCCC}
%    \toprule
%    Protocol            & Number of Ids & Comm. Rounds & Comm. Data (kB.) & Throughput (ops/s) \\
%  \midrule
%    CBC-MAC-AES & 1  & XXX & XXX & XXX \\ % c =  2, b =  3
%    HtMAC-MiMC  & 1  & XXX  & XXX & XXX \\
%  \midrule
%    CBC-MAC-AES & 2  & XXX & XXX & XXX \\ % c =  2, b =  3
%    HtMAC-MiMC  & 2  & XXX & XXX & XXX \\
%
%  \midrule
%    CBC-MAC-AES & 4 & XXX &  XXX & XXX \\ % c =  2, b =  3
%    HtMAC-MiMC  & 4 & XXX  & XXX & XXX \\
%
%  \midrule
%    CBC-MAC-AES & 256  & XXX &  XXX & XXX \\ % c =  2, b =  3
%    HtMAC-MiMC  & 256  & XXX & XXX & XXX \\
%
%   \midrule
%    CBC-MAC-AES & 512 & XXX &  XXX & XXX \\ % c =  2, b =  3
%    HtMAC-MiMC  & 512 & XXX & XXX & XXX \\
%
%    \midrule
%    CBC-MAC-AES & 1024 & XXX &  XXX & XXX \\ % c =  2, b =  3
%    HtMAC-MiMC  & 1024 & XXX & XXX & XXX \\
% 
%    \bottomrule
%  \end{tabularx}}
%  \caption {50Mb/s WAN experiments for three party RSS access token generation}
%  \label{tab:dabit}
%\end{center}
%\end{table*}

